Alleviating Catastrophic Forgetting in Facial Expression Recognition with Emotion-Centered Models

Facial expression recognition is a pivotal component in machine learning, facilitating various applications. However, convolutional neural networks (CNNs) are often plagued by catastrophic forgetting, impeding their adaptability. The proposed method, emotion-centered generative replay (ECgr), tackles this challenge by integrating synthetic images from generative adversarial networks. Moreover, ECgr incorporates a quality assurance algorithm to ensure the fidelity of generated images. This dual approach enables CNNs to retain past knowledge while learning new tasks, enhancing their performance in emotion recognition. The experimental results on four diverse facial expression datasets demonstrate that incorporating images generated by our pseudo-rehearsal method enhances training on the targeted dataset and the source dataset while making the CNN retain previously learned knowledge.

==> backup-plots.tex <==
% figura com o gráfico principal da mug
% com linhas em volta e legenda separada
\begin{figure}
    \centering
    \begin{tikzpicture}[scale=0.85]
        \begin{axis}[
            %xlabel={Datasets},
            ylabel={Accuracy},
            legend pos=outer north east,
            xtick=data,
            xticklabels={Baseline, JAFFE, TFEID, CK+},
            ]
            \addplot[color=blue,mark=*] coordinates {
                (1, 0.9800)
                (2, 1.0000)
                (3, 1.0000)
                (4, 1.0000)
            };
            \addlegendentry{Joint}
            
            \addplot[color=purple,mark=x] coordinates {
                (1, 0.9800)
                (2, 0.7500)
                (3, 0.7100)
                (4, 0.6300)
            };
            \addlegendentry{Fine-tune}
            
            \addplot[color=green,mark=triangle] coordinates {
                (1, 0.9800)
                (2, 0.8800)
                (3, 0.8400)
                (4, 0.8500)
            };
            \addlegendentry{ECgr}
            
            \addplot[color=red,mark=square] coordinates {
                (1, 0.9800)
                (2, 0.9300)
                (3, 0.8700)
                (4, 0.8700)
            };
            \addlegendentry{ECgr+QA}
            
            \addplot[color=black,mark=diamond] coordinates {
                (1, 0.9800)
                (2, 0.9400)
                (3, 0.7800)
                (4, 0.7300)
            };
            \addlegendentry{ECgr+wQA}
        \end{axis}
    \end{tikzpicture}
    \caption{Accuracy results on the MUG dataset, showcasing the continuous adaptation of a trained CNN across JAFFE, TFEID, and CK+ datasets relative to the baseline accuracy.}
    \label{results:accuracy_mug}
\end{figure}

% figura com o gráfico principal da mug
% cores originais do plot
\begin{figure}
    \centering
    \begin{tikzpicture}[scale=1]
        \begin{axis}[
            clip=false,
            ylabel={Accuracy},
            ymin=0.6,
            %legend pos=outer north east,
            xtick=data,
            xticklabels={Baseline, JAFFE, TFEID, CK+},
            ytick={0.6, 0.65, 0.7, 0.75, 0.8, 0.85, 0.9, 0.95, 1},
            axis lines=left,
            xmajorgrids=true,
            ymajorgrids=true,
            grid style=dashed,
            ]
            \addplot[color=blue,mark=*] coordinates {
                (1, 0.9800)
                (2, 1.0000)
                (3, 1.0000)
                (4, 1.0000)
            }node[right, pos=1.03]{Joining datasets};
            %\addlegendentry{Joint}
            
            \addplot[color=purple,mark=x] coordinates {
                (1, 0.9800)
                (2, 0.7500)
                (3, 0.7100)
                (4, 0.6300)
            }node[right, pos=1.03]{Fine-tuning};
            %\addlegendentry{Fine-tune}
            
            \addplot[color=green,mark=triangle] coordinates {
                (1, 0.9800)
                (2, 0.8800)
                (3, 0.8400)
                (4, 0.8500)
            }node[right, pos=1.03]{ECgr};;
            %\addlegendentry{ECgr}
            
            \addplot[color=red,mark=square] coordinates {
                (1, 0.9800)
                (2, 0.9300)
                (3, 0.8700)
                (4, 0.8700)
            }node[right, pos=1.03]{ECgr+QA};;
            %\addlegendentry{ECgr+QA}
            
            \addplot[color=black,mark=diamond] coordinates {
                (1, 0.9800)
                (2, 0.9400)
                (3, 0.7800)
                (4, 0.7300)
            }node[right, pos=1.03]{ECgr+wQA};;
            %\addlegendentry{ECgr+wQA}
        \end{axis}
    \end{tikzpicture}
    \caption{Accuracy results on the MUG dataset, showcasing the continuous adaptation of a trained CNN across JAFFE, TFEID, and CK+ datasets relative to the baseline accuracy.}
    \label{results:accuracy_mug}
\end{figure}

% figura com os gráficos da jaffe e tfeid
\begin{figure}
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                width=\textwidth, % Set the width of the plot to match the subfigure
                %xlabel={Datasets},
                ylabel={Accuracy},
                %legend pos=north west, % Move the legend to the top left corner
                xtick=data,
                xticklabels={Baseline, TFEID, CK+},
                ]
                \addplot[color=blue,mark=*] coordinates {
                    (1, 0.7800)
                    (2, 0.9400)
                    (3, 0.9900)
                };
                %\addlegendentry{Joint}
                
                \addplot[color=purple,mark=x] coordinates {
                    (1, 0.7800)
                    (2, 0.7600)
                    (3, 0.5700)
                };
                %\addlegendentry{Fine-tune}
                
                \addplot[color=green,mark=triangle] coordinates {
                    (1, 0.7800)
                    (2, 0.6400)
                    (3, 0.6100)
                };
                %\addlegendentry{ECgr}
                
                \addplot[color=red,mark=square] coordinates {
                    (1, 0.7800)
                    (2, 0.6200)
                    (3, 0.5500)
                };
                %\addlegendentry{ECgr+QA}
                
                \addplot[color=black,mark=diamond] coordinates {
                    (1, 0.7800)
                    (2, 0.6900)
                    (3, 0.5900)
                };
                %\addlegendentry{ECgr+wQA}
            \end{axis}
        \end{tikzpicture}
        \caption{Results for the JAFFE dataset}
        \label{results:accuracy_jaffe}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                width=\textwidth, % Set the width of the plot to match the subfigure
                %xlabel={Datasets},
                %ylabel={Accuracy},
                legend pos=outer north east, % Move the legend to the top left corner
                %legend style={at={(-0.5,-0.15)},anchor=north,legend columns=5},
                xtick=data,
                xticklabels={Baseline, CK+},
                ]
                \addplot[color=blue,mark=*] coordinates {
                    (1, 0.7400)
                    (2, 1.0000)
                };
                \addlegendentry{Joint}
                
                \addplot[color=purple,mark=x] coordinates {
                    (1, 0.7400)
                    (2, 0.4900)
                };
                \addlegendentry{Fine-tune}
                
                \addplot[color=green,mark=triangle] coordinates {
                    (1, 0.7400)
                    (2, 0.6200)
                };
                \addlegendentry{ECgr}
                
                \addplot[color=red,mark=square] coordinates {
                    (1, 0.7400)
                    (2, 0.7600)
                };
                \addlegendentry{ECgr+QA}
                
                \addplot[color=black,mark=diamond] coordinates {
                    (1, 0.7400)
                    (2, 0.7000)
                };
                \addlegendentry{ECgr+wQA}
            \end{axis}
        \end{tikzpicture}
        \caption{Results for the TFEID dataset}
        \label{results:accuracy_tfeid}
    \end{subfigure}
    \caption{Accuracy comparison for the JAFFE and TFEID datasets.}
    \label{results:jaffe_tfeid_accuracy}
\end{figure}
